MMBench: Is Your Multi-modal Model an All-around Player?

Large vision-language models (VLMs) have recently achieved remarkable progress, exhibiting impressive multimodal perception and reasoning abilities. However, effectively evaluating these large VLMs remains a major challenge, hindering future development in this domain. Traditional benchmarks like VQAv2 or COCO Caption provide quantitative performance measurements but lack fine-grained ability assessment and robust evaluation metrics. Meanwhile, subjective benchmarks, such as OwlEval, offer comprehensive evaluations of a model's abilities by incorporating human labor, which is not scalable and may display significant bias. In response to these challenges, we propose MMBench, a bilingual benchmark for assessing the multi-modal capabilities of VLMs. MMBench methodically develops a comprehensive evaluation pipeline, primarily comprised of the following key features: 1. MMBench is meticulously curated with well-designed quality control schemes, surpassing existing similar benchmarks in terms of the number and variety of evaluation questions and abilities; 2. MMBench introduces a rigorous CircularEval strategy and incorporates large language models to convert free-form predictions into pre-defined choices, which helps to yield accurate evaluation results for models with limited instruction-following capabilities. 3. MMBench incorporates multiple-choice questions in both English and Chinese versions, enabling an apples-to-apples comparison of VLMs' performance under a bilingual context. To summarize, MMBench is a systematically designed objective benchmark for a robust and holistic evaluation of vision-language models. We hope MMBench will assist the research community in better evaluating their models and facilitate future progress in this area. The evalutation code of MMBench has been integrated into VLMEvalKit: https://github.com/open-compass/VLMEvalKit.

==> figure/1-mm_ability.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{pdf/2-ability-dist.pdf}
\vspace{-0.2em}
\caption{\textbf{Overview of existing ability dimensions in \ourmethod.} 
Currently, \ourmethod incorporates three levels of ability dimensions (from L-1 to L-3), which encompass 20 distinct leaf abilities. 
Note that the demonstrated ability taxonomy is an initial version.
Further adjustments can be made to improve the taxonomy and make it more comprehensive. 
% It is important to note that these ability dimensions are dynamic, not static. They are subject to expansion as we continuously work on it. 
% \textbf{Fine-grained-S} perception refers to fine-grained single instance perception, and \textbf{Fine-grained-C} perception refers to fine-grained cross instance perception.}
}
\label{fig:1-mm_ability}
\vspace{-3mm}
\end{figure}


==> figure/2-ability-dist.tex <==
\label{method:statistics}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pdf/2-ability-dist.pdf}
\caption{\textbf{Data distribution of L-1 to L-3 ability dimensions of \ourmethod.} We show the number of these data samples belonging to each ability in the bracket.}
\label{fig:data_statistics}
\end{figure}


==> figure/ability_performance.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\linewidth]{pdf/1-ability-performance.pdf}
\vspace{-0.6em}
\caption{\textbf{Results of six representative large vision-language models across the 20 ability dimensions defined in MMBench.} For more comprehensive evaluation results on additional models, please refer to \Cref{tab:main_results_short} and \Cref{tab:main_results_short_dev}, as well as the appendix.}
\label{fig:0-ability-performance}
\end{figure}

